Adaptive optics and lightcurve data of asteroids: twenty shape models and information content analysis

We present shape models and volume estimates of twenty asteroids based on relative photometry and adaptive optics images. We discuss error estimation and the effects of myopic deconvolution on shape solutions. For further analysis of the information capacities of data sources, we also present and discuss ambiguity and uniqueness results for the reconstruction of nonconvex shapes from photometry.

==> tabs/tab1_old.tex <==
\onecolumn
%\longtab{
\begin{longtable}{r@{\,\,\,}l rrrr rrr rr}
\caption{\label{tab:results}Rotation state parameters $\lambda_{\mathrm{a}}$, $\beta_{\mathrm{a}}$, $P_{\mathrm{a}}$ with a reference to the corresponding publication that we used as initial inputs for the modeling with ADAM, rotation state parameters $\lambda$, $\beta$, $P$ derived by the ADAM algorithm, and the number of available light curves $N_{\mathrm{lc}}$ and disk-resolved images $N_{\mathrm{ao}}$.}\\
\hline 
\multicolumn{2}{c} {Asteroid} & \multicolumn{1}{c} {$\lambda_{\mathrm{a}}$} & \multicolumn{1}{c} {$\beta_{\mathrm{a}}$} & \multicolumn{1}{c} {$P_{\mathrm{a}}$} & \multicolumn{1}{c} {Reference} & \multicolumn{1}{c} {$\lambda$} & \multicolumn{1}{c} {$\beta$} & \multicolumn{1}{c} {$P$} & \multicolumn{1}{c} {$N_{\mathrm{lc}}$} & \multicolumn{1}{c} {$N_{\mathrm{ao}}$} \\
\multicolumn{2}{l} {} & [deg] & [deg] & \multicolumn{1}{c} {[hours]} &  & [deg] & [deg] & \multicolumn{1}{c} {[hours]} &  & \\
\hline\hline

\endfirsthead
\caption{continued.}\\

\hline
\multicolumn{2}{c} {Asteroid} & \multicolumn{1}{c} {$\lambda_{\mathrm{a}}$} & \multicolumn{1}{c} {$\beta_{\mathrm{a}}$} & \multicolumn{1}{c} {$P_{\mathrm{a}}$} & \multicolumn{1}{c} {Reference} & \multicolumn{1}{c} {$\lambda$} & \multicolumn{1}{c} {$\beta$} & \multicolumn{1}{c} {$P$} & \multicolumn{1}{c} {$N_{\mathrm{lc}}$} & \multicolumn{1}{c} {$N_{\mathrm{ao}}$} \\
\multicolumn{2}{l} {} & [deg] & [deg] & \multicolumn{1}{c} {[hours]} &  & [deg] & [deg] & \multicolumn{1}{c} {[hours]} &  & \\
\hline\hline
\endhead
\hline
\endfoot
\hline
  7 &         Iris &   16 &  15   & 7.138843 &  \citet{Kaasalainen2002b} &   18$\pm$4 &  19$\pm$4 & 7.138843 &  39 & 14 \\
  7 &         Iris &  196 &   2   & 7.138843 &  \citet{Kaasalainen2002b} &    \multicolumn{3}{c} {Rejected} &  39 & 14 \\
 12 &     Victoria &  174 & $-$17 & 8.66034 &        \citet{Hanus2016a} &  177$\pm$4 & $-$34$\pm$4 & 8.66034 &  53 &  8 \\
 14 &        Irene &   95 & $-$11 & 15.02986 &         \citet{Hanus2011} &   91$\pm$7 & $-$14$\pm$4 & 15.02988 &  29 &  3 \\
 15 &      Eunomia &    3 & $-$67 & 6.082753 &  \citet{Kaasalainen2002b} &    0$\pm$5 & $-$67$\pm$2 & 6.082752 &  48 &  8 \\
 23 &       Thalia &  159 & $-$45 & 12.31241 &        \citet{Torppa2003} &  158$\pm$2 & $-$45$\pm$4 & 12.31241 &  50 &  2 \\
 23 &       Thalia &  343 & $-$69 & 12.31241 &        \citet{Torppa2003} &  341$\pm$3 & $-$73$\pm$6 & 12.31241208 &  50 &  2 \\
 24 &       Themis &  137 &  59   & 8.374187 &        \citet{Hanus2016a} &  138$\pm$4 &  69$\pm$5 & 8.374187 &  46 &  4 \\
 24 &       Themis &  331 &  52   & 8.374187 &        \citet{Hanus2016a} &  328$\pm$5 &  70$\pm$2 & 8.374187 &  46 &  4 \\
 28 &      Bellona &  102 &  $-$8 & 15.70785 &        \citet{Durech2011} &  99$\pm$4 &  $-$16$\pm$6 & 15.70785 &  23 &  1 \\
 40 &     Harmonia &   22 &  31   & 8.908483 &         \citet{Hanus2011} &   22$\pm$2 &  38$\pm$5 & 8.908485 &  23 &  3 \\
 42 &         Isis &  106 &  40   & 13.58364 &         \citet{Hanus2011} &  108$\pm$1 &  47$\pm$3 & 13.58364 &  31 &  1 \\
 48 &        Doris &  108 &  47   & 11.8901 &        \citet{Hanus2016a} &    \multicolumn{3}{c} {Rejected} &  31 &  2 \\
 48 &        Doris &  297 &  61   & 11.8901 &        \citet{Hanus2016a} &  296$\pm$3 &  57$\pm$5 & 11.89010 &  31 &  2 \\
 56 &       Melete &  103 & $-$27 & 18.14817 &        \citet{Hanus2016a} &  103$\pm$1 & $-$26$\pm$2 & 18.14817 &  34 &  2 \\
 56 &       Melete &  282 &  $-$5 & 18.14817 &        \citet{Hanus2016a} &  283$\pm$1 &  $-$3$\pm$3 & 18.14817 &  34 &  2 \\
 65 &       Cybele &  208 &  $-$7 & 6.081434 &        \citet{Franco2015} &  208$\pm$1 &  $-$3$\pm$3 & 6.081435 &  59 &  7 \\
 65 &       Cybele &   27 & $-$14 & 6.081434 &        \citet{Franco2015} &    \multicolumn{3}{c} {Rejected} &  59 &  7 \\
 72 &      Feronia &  102 & $-$55 & 8.09068 &        \citet{Hanus2013a} &  100$\pm$6 & $-$51$\pm$6 & 8.09068 &  20 &  2 \\
121 &     Hermione &    4 &  13   & 5.550878 &      \citet{Descamps2009} &  362$\pm$2 &   13$\pm$1 & 5.550877 &  48 & 13 \\
146 &       Lucina &  305 & $-$41 & 18.5539 &        \citet{Durech2009} &  304$\pm$6 & $-$41$\pm$2 & 18.55387 &  22 &  2 \\
250 &      Bettina &  100 &  17   & 5.054420 &        \citet{Torppa2003} &  101$\pm$2 &  9$\pm$2 & 5.054414 &  22 &  1 \\
283 &         Emma &  251 &  22   & 6.895222 &   \citet{Michalowski2006} &  256$\pm$3 &  23$\pm$3 & 6.89523 &  29 &  5 \\
283 &         Emma &   85 &  37   & 6.895221 &   \citet{Michalowski2006} &    \multicolumn{3}{c} {Rejected} &  29 &  5 \\
354 &     Eleonora &  144 &  54   & 4.277186 &         \citet{Hanus2011} &  161$\pm$8 &  41$\pm$7 & 4.277186 &  64 &  3 \\
511 &       Davida &  297 &  26   & 5.129363 &        \citet{Torppa2003} &  299$\pm$1 &  24$\pm$1 & 5.129363 &  58 & 10 \\
1036 &      Ganymed &  190 & $-$78 & 10.31284 &       \citet{Hanus2015a} &  198$\pm$10 & $-$79$\pm$1 & 10.31304 & 177 &  5 \\
\hline
\end{longtable}
%\tablefoot{
%The table gives ecliptic coordinates $\lambda_{\mathrm{a}}$ and $\beta_{\mathrm{a}}$ and sidereal rotation period $P_{\mathrm{a}}$ of the previously published solution, which was used an an input for the shape modeling by ADAM, the reference to this solution, previous size (diameter) estimate $D_\mathrm{p}$ and its reference, ecliptic coordinates $\lambda$ and $\beta$, sidereal rotation period $P$ and volume-equivalent diameter $D$ of the shape solution derived here by ADAM, adopted mass $M$ and its reference, derived density $\rho$ and the Tholen ($T_1$) and Bus-DeMeo ($T_1$) taxonomic classification.}
%}
\twocolumn


==> tabs/tab2_old.tex <==
\onecolumn
%\scriptsize{
%\longtab{
%\begin{tabular}{r@{\,\,\,}l lc| r@{\,\,\,}l lc} \hline
% \multicolumn{2}{c} {Asteroid} & Date & Observer &  \multicolumn{2}{c}{Asteroid} & Date & Observer\\ \hline\hline
\begin{longtable}{r@{\,\,\,}l cc c cc cc c}
\caption{\label{tab:densities}Bulk density estimates based on our volume estimated by the ADAM shape modeling from combined optical light curves, disk-resolved images and stellar occultations.}\\
\hline
 \multicolumn{2}{c} {Asteroid} & $D_{\mathrm{a}}$ & Reference & $D$ & $M$ & Reference & T1 & T2 & $\rho$ \\
 \multicolumn{2}{c} {} & [km] &  & [km] & [10$^{18}$ kg] &  &  &  &  [gcm$^{-3}$] \\ \hline\hline

\endfirsthead
\caption{continued.}\\

\hline
 \multicolumn{2}{c} {Asteroid} & $D_{\mathrm{a}}$ & Reference & $D$ & $M$ & Reference & T1 & T2 & $\rho$ \\
 \multicolumn{2}{c} {} & [km] &  & [km] & [10$^{18}$ kg] &  &  &  &  [gcm$^{-3}$] \\ \hline\hline
\endhead
\hline
\endfoot
  7 &         Iris &  203$\pm$24 &        \citet{Hanus2013b} &   216$\pm$7 &  12.9$\pm$2.1 &        \citet{Carry2012b} &  S &  S & 2.4$\pm$0.5 \\
  7 &         Iris &  203$\pm$24 &        \citet{Hanus2013b} &      \multicolumn{6}{c} {Rejected} \\
 12 &     Victoria &  124$\pm$8 &        \citet{Carry2012b} &   115$\pm$3 &  2.5$\pm$0.5 &        \citet{Carry2012b} &  S &  L & 3.1$\pm$0.6 \\
 14 &        Irene &  149$\pm$17 &        \citet{Hanus2013b} &   155$\pm$6 &  2.8$\pm$1.0 &        \citet{Fienga2014} &  S &  S & 1.4$\pm$0.5 \\
 15 &      Eunomia &  254$\pm$27 &        \citet{Hanus2013b} &   275$\pm$5 &  31.4$\pm$1.8 &        \citet{Carry2012b} &  S &  S & 2.9$\pm$0.2 \\
 23 &       Thalia &  107$\pm$12 &        \citet{Hanus2013b} &   120$\pm$8 &  2.0$\pm$0.1 &        \citet{Carry2012b} &  S &  S & 2.2$\pm$0.4 \\
 23 &       Thalia &  107$\pm$12 &        \citet{Hanus2013b} &   120$\pm$8 &  2.0$\pm$0.1 &        \citet{Carry2012b} &  S &  S & 2.2$\pm$0.4 \\
 24 &       Themis &  184$\pm$11 &        \citet{Carry2012b} &   215$\pm$15 &  5.9$\pm$1.9 &        \citet{Carry2012b} &  C &  B & 1.1$\pm$0.4 \\
 24 &       Themis &  184$\pm$11 &        \citet{Carry2012b} &   215$\pm$15 &  5.9$\pm$1.9 &        \citet{Carry2012b} &  C &  B & 1.1$\pm$0.4 \\
 28 &      Bellona &  121$\pm$11 &        \citet{Hanus2013b} &   135$\pm$7 &  2.6$\pm$0.1 &        \citet{Carry2012b} &  S &  S & 2.0$\pm$0.3 \\
 40 &     Harmonia &  123$\pm$12 &        \citet{Hanus2013b} &   113$\pm$7 &    &                     &  S &  S &   \\
 42 &         Isis &   97$\pm$10 &        \citet{Hanus2013b} &   102$\pm$4 &  1.6$\pm$0.5 &        \citet{Carry2012b} &  S &  L & 2.8$\pm$1.0 \\
 48 &        Doris &  212$\pm$11 &        \citet{Carry2012b} &      \multicolumn{6}{c} {Rejected} \\
 48 &        Doris &  212$\pm$11 &        \citet{Carry2012b} &   223$\pm$23 &  6.1$\pm$3.0 &        \citet{Carry2012b} & CG & Ch & 1.1$\pm$0.6 \\
 56 &       Melete &  114$\pm$8 &        \citet{Carry2012b} &   119$\pm$5 &  4.6$\pm$1.0 &        \citet{Carry2012b} &  P & Xk & 5.2$\pm$1.3 \\
 56 &       Melete &  114$\pm$8 &        \citet{Carry2012b} &   119$\pm$5 &  4.6$\pm$1.0 &        \citet{Carry2012b} &  P & Xk & 5.2$\pm$1.3 \\
 65 &       Cybele &  248$\pm$18 &        \citet{Carry2012b} &   296$\pm$25 &  13.6$\pm$3.1 &        \citet{Carry2012b} &  P & Xc & 1.0$\pm$0.3 \\
 65 &       Cybele &  248$\pm$18 &        \citet{Carry2012b} &      \multicolumn{6}{c} {Rejected} \\
 72 &      Feronia &   74$\pm$6 &        \citet{Hanus2013b} &    84$\pm$10 &  3.3$\pm$8.5 &        \citet{Carry2012b} & TDG &  $-$ & $-$ \\
121 &     Hermione &  187$\pm$6 &      \citet{Descamps2009} &   196$\pm$15 &  5.0$\pm$0.3 &        \citet{Carry2012b} &  C & Ch & 1.26$\pm$0.30 \\
146 &       Lucina &  119$\pm$11 &        \citet{Hanus2013b} &   131$\pm$15 &   &                   &  C & Ch &   \\
250 &      Bettina &  119$\pm$11 &        \citet{Hanus2013b} &   109$\pm$5 &    &                  &  M & Xk &   \\
283 &         Emma &  133$\pm$10 &        \citet{Carry2012b} &   142$\pm$14 &  1.4$\pm$0.0 &      \citet{Marchis2008a} &  X &  C & 0.9$\pm$0.3 \\
283 &         Emma &  133$\pm$10 &        \citet{Carry2012b} &      \multicolumn{6}{c} {Rejected} \\
354 &     Eleonora &  154$\pm$6 &        \citet{Carry2012b} &   169$\pm$30 &  7.2$\pm$2.6 &        \citet{Carry2012b} &  S & Sl & 2.8$\pm$1.8 \\
511 &       Davida &  289$\pm$21 &        \citet{Conrad2007} &   311$\pm$5 &  33.7$\pm$5.7 &        \citet{Fienga2014} &  C &  C & 2.1$\pm$0.4 \\
1036 &      Ganymed &  36$\pm$3 &         \citet{Hanus2015a} &    38$\pm$3 &  0.15$\pm$0.12 &             Fienga, privat com. &  S &  S & 5.2$\pm$4.4 \\
\hline
\end{longtable}
\tablefoot{
The table gives previous size (surface- or volume-equivalent diameter) estimate $D_\mathrm{a}$ and its reference, volume-equivalent diameter $D$ of the shape solution derived here by ADAM, adopted mass $M$ and its reference, the Tholen \citep[T1,][]{Tholen1989, Tholen1989b} and SMASS II \citep[T2,][]{Bus2002} taxonomic classes, and our density determination $\rho$.}
%}
%}
\twocolumn
